A Simple Approach to Case-Based Reasoning in Knowledge Bases

We present a surprisingly simple yet accurate approach to reasoning in knowledge graphs (KGs) that requires \emph{no training}, and is reminiscent of case-based reasoning in classical artificial intelligence (AI). Consider the task of finding a target entity given a source entity and a binary relation. Our non-parametric approach derives crisp logical rules for each query by finding multiple \textit{graph path patterns} that connect similar source entities through the given relation. Using our method, we obtain new state-of-the-art accuracy, outperforming all previous models, on NELL-995 and FB-122. We also demonstrate that our model is robust in low data settings, outperforming recently proposed meta-learning approaches

==> sections/analysis.tex <==
\subsection{NELL}
As seen in table \ref{tab:larger3}, CBR outperforms previous approaches on the NELL-995 dataset by a huge margin. In this section we investigate this high performance when compared to several other methods.
On detailed investigation we notice that CBR overwhelmingly outperforms MINERVA \cite{das2018go} on generic relations in NELL-995. For example, the relation \fontsf{agent_belongs_to_organization} connects a diverse set of entities. This is better described in figure \ref{fig}. MINERVA aims to learn a policy to find a reasoning path that is able to generalize to all these examples. As MINERVA ignores the query entity and relies on the query relation, it fails to generalize well to all the types of entities in the \fontsf{agent_belongs_to_organization} relation in the NELL-995 graph.
CBR, is able to handle this problem as instead of learning rules from the entire train set it learns and applies rules from the closest entities to the question entity. 
As in the example in Fig \ref{fig}, CBR is able to handle the question (Montreal \fontsf{Canadiens, agent_belongs_to_organization}, ?) by retrieving nearest neighbors which are other sports teams which belong to leagues.
This allows CBR to better generalize to a diverse set of query entities as unlike MINERVA it does not try to generalize all of the reasoning rules within its parameters. 

